Towards Using Package Centrality Trend to Identify Packages in Decline

Due to their increasing complexity, today's software systems are frequently built by leveraging reusable code in the form of libraries and packages. Software ecosystems (e.g., npm) are the primary enablers of this code reuse, providing developers with a platform to share their own and use others' code. These ecosystems evolve rapidly: developers add new packages every day to solve new problems or provide alternative solutions, causing obsolete packages to decline in their importance to the community. Developers should avoid depending on packages in decline, as these packages are reused less over time and may become less frequently maintained. However, current popularity metrics (e.g., Stars, and Downloads) are not fit to provide this information to developers because their semantics do not aptly capture shifts in the community interest. In this paper, we propose a scalable approach that uses the package's centrality in the ecosystem to identify packages in decline. We evaluate our approach with the npm ecosystem and show that the trends of centrality over time can correctly distinguish packages in decline with an ROC-AUC of 0.9. The approach can capture 87% of the packages in decline, on average 18 months before the trend is shown in currently used package popularity metrics. We implement this approach in a tool that can be used to augment the npms metrics and help developers avoid packages in decline when reusing packages from npm.

==> discussion.tex <==
In this section, we dive into two unexplored aspects of centrality and our approach. 
First, we conduct a preliminary analysis on how centrality ranking compares to the ranking of packages yielded by the JavaScript survey.
Then, we investigate if our approach, using the centrality trend, could detect deprecated package earlier than currently used metrics. 




\subsection{Comparing the centrality ranking with the State of JavaScript rankings}


We want to investigate the relationship between the package centrality in the \npm ecosystem and how the \npm community perceives the packages over time.
We intuitively expect the centrality to capture the importance of a package in \npm ecosystem. 
The most central packages are depended upon by thousands of other packages and JavaScript projects, which indicates their popularity and recognition in the community.
However, how does the JavaScript community perceives highly central packages?
Is the ranking we obtain using the centrality metric more related to the community interest, awareness or satisfaction when using these packages?
Answering such questions will helps us interpret the implication of a consistent centrality decrease.


To investigate how the JavaScript community perceives a software package and its association with the package centrality, we need the opinions of a vast number of JavaScript developers.
For this aim, we use the data from the State of JavaScript survey, the most extensive survey on the JavaScript ecosystem.
As described in \Cref{sub:data_survey}, the survey asks JavaScript developers about their opinion on popular \npm packages.
Based on the responses, each package is ranked according to four categories: satisfaction, interest, awareness, and usage.
The satisfaction ranking, for instance, ranks packages based on the share of satisfied respondents, from highest (first) to lowest (last). 



We collect the responses data from four yearly versions of the survey: 2016, 2017, 2018, and 2019 where a survey compose 21 packages, 30 packages, 24 packages, and	28 packages, respectively.
We assign for each package from each survey version the centrality ranking at the time the survey was first open to the public. 
Then, we use the Normalized Discounted Cumulative Gain (NDCG) method to measure the centrality rankings' relevance to each of the survey ranking categories. NDCG is a popular method for measuring the relevancy of a ranking set and used previously including in software engineering research in the context of ranking \npm packages~\cite{Jarvelin_TOIS2002, Wang_PMLR2013, McSherry_ECIR2008, Abdellatif_IST2020}. NDCG takes as input ranking values of two list: the proposed ranking and the ground truth ranking. In our study, we consider our ranking based on the centrality as the proposed ranking, and the other four criteria of ranking from developers as ground truth ranking. We basically compare the centrality ranking to the ranking State of JavaScript survey produced for satisfaction, interest, awareness, and usage.
A NDCG score ranges between 0 to 1 and is used typically to measure ranking quality, with higher values indicating a ranking closer to the ideal ranking (ground-truth).




\Cref{fig:heatmap_survey_ndcg} shows a heatmap representing the results of NDCG for comparing the centrality rankings to each survey category across the  four survey versions.
Darker colors represent a higher relevance score between the survey category ranking and the centrality ranking.
The figure shows that the centrality rankings have the highest NDCG scores when associating them with the satisfaction ranking across all survey versions (2016 to 2019).
This result indicates that the centrality ranking might be considered as an indicator of the satisfaction developers have with using a package. 
A package with a higher centrality ranking indicates that developers both use the package and are satisfied with it, reporting they will tend continue to use it in the feature instead of searching for other solutions.
The second highest NDCG score was obtained with the awareness ranking. 
A highly central package is likely to be known by a significant share of the community; which endorse centrality as a good popularity metric.


The ranking with the lowest NDCG score, and therefore the most distinct to the ranking centrality yields, is the usage rankings. 
A possible explanation is that the usage ranking focus on assessing if developers have used the package anytime in the past, which is different from whether developers are currently using the package in their projects. 
More importantly, the usage ranking does not cover if developers have any positive or negative opinion about the packages they used.
This is further corroborated by the contrast between the NDCG scores obtained comparing the centrality ranking with the satisfaction and the usage rankings. 
We believe that the centrality and satisfaction rankings are more likely to capture if developers are currently using a package than the usage rankings.

This analysis indicates that centrality is better at capturing the satisfaction of JavaScript developers towards popular packages than their past usage.
However, while the survey data provides us with an invaluable dataset with the opinion of thousands of JavaScript developers, our analysis should be interpreted as preliminary. 
The survey data contains assessments of just a very small number of packages (approximately 30 packages per survey), and further studies are required to validate if centrality is a good indicator of user satisfaction of JavaScript packages. 













\begin{figure}[t]
    \centering
    \includegraphics[trim=0 .25in 0 .21in, clip,width=\linewidth]{figs/heatmap_survey_ndcg.pdf}
    \caption{Heatmap of NDCG scores measuring the relevancy of centrality ranking to the Sate of JavaScript surveys' rankings.}
    \label{fig:heatmap_survey_ndcg}
\end{figure}


















\subsection{Does our approach detect packages \decline earlier using the trend of other metrics other than centrality?}



In RQ3, we showed that centrality and current popularity metrics, such as the number of downloads and stars, are not correlated for the majority of packages.
Hence, a package's centrality trend can provide new insights if provided to developers.
In this subsection, we want to know if these other metrics could be still used to detect packages that have been deprecated by their maintainers. 
Deprecated packages are extreme cases of a packages \decline, where maintainers (for a variety of reasons) have made the conscious effort to stop maintaining the package. 
Hence, it is crucial that developers are aware of packages \decline as early as possible, to prevent them from depending on source code that is not properly maintained.


We want to evaluate if currently used popularity metrics such as the number of downloads, dependents, stars and forks, can detect deprecated packages earlier than the centrality.
We replicate the method we used (detailed in \Cref{sub:detect_decline}) to identify if a trend is significantly declining for the four popularity metrics, which we will refer in this section as the \textit{slope analysis}. 
The slope analysis consists in calculating the slope of the trend using the least-squares regression~\cite{Handbook:online} and testing if the slope is significant using the Wald Test~\cite{Judge_Book1985}.
A significant negative slope on a period of six months classifies a package \decline.
We run this slope analysis using one of the popularity metrics to detect a package \decline, initially before the depreciation date. 
If the decline is detected, we apply a window sliding approach explained in \nameref{rq:two:num} to measure how early the slope analysis can detect packages \decline using that metric.
We define the point in which the slope analysis identifies the package \decline as the \textit{detection time}. 
In contrast, if the slope analysis does not detect the decline, we invert the window sliding approach to measure how late it can detect the package \decline (after the deprecation date) using that metric.
In this case, the \textit{detection time} will occur after the deprecation date.
Finally, to compare how early each approach can identify packages \decline, we compare the detection time of our approach against the detection time yielded by the slope analysis with each popularity metric.
We refer to the difference between the centrality detection time and the slope analysis detection time as the \textit{time latency}. 


\Cref{tab:time_metrics_to_centrality} show the results of this analysis, always comparing the four popularity metrics with our approach that uses centrality. 
First, we show in the column ``Total Cases" the number of packages in which we could retrieve the necessary data for this analysis. Due to the limitation of retrieving the history of the stars and forks, we analyzes only 203 and 174 packages, respectively. 
The column ``\# Detected (\%)" shows how many packages each metric could detect as decline either before or after the deprecation date. 
We can observe that our approach was able to detect a decline in centrality in 95\% of the deprecated packages, while only 5\% of the packages have shown a decline in the number of dependents and downloads. 
Surprisingly, we find that 50\% of the deprecated packages have shown a decrease in the number of stars and 57\% have exhibited a decrease in the number of forks. 


The group of columns ``Detected Before Centrality" showcase the number packages that the slope analysis with each popularity metric was able to identify the decline before centrality (``\# Detected") and their average and median time latency.  
We found that the number of dependents could not identify any package \decline before centrality, and other metrics such as Stars and Forks were able to identify 19 and 20 packages before centrality.
In such cases, the stars and forks decreased in median 4-5 months before the centrality of the package declined (see Time Latency column).


Similarly, we show in the group of columns ``Detected After Centrality" the number of deprecated packages the slope analysis were able to identify after the centrality approach. 
The majority of packages \decline were only identified after their centrality showed a clear decline.
For instance, the 28 packages detected by the number dependents only showed a substantial decrease in the number of dependents 16 months after the centrality decreased (see the ``Time Latency" column). 
The number of stars and forks showed similar results, with approximately 80 packages exhibiting a drop in the number of stars/forks only 9 to 13 months after their centrality decreased. 

Finally, we show the overall results in the column ``Overall Latency", where we present the mean and median time latency between our approach and the slope analysis for all metrics.
All popularity metrics have identified the majority of packages \decline after the centrality approach with considerable average latency between 10 months (Forks) to 16 months (Dependents).
This analysis indicates that, in most cases, centrality can identify packages \decline earlier than currently used popularity metrics. 
However, we also identified a few packages in which current popularity metrics (stars and forks) can also decrease before the package's centrality. 



\begin{table*}
    \centering
    \caption{Performance of our approach using the centrality comparing to the usage of other metrics.}
    \label{tab:time_metrics_to_centrality}
    \input{tables/time_metrics_to_centrality}
\end{table*}















